Learning Domain Specific Language Models for Automatic Speech Recognition through Machine Translation

Automatic Speech Recognition (ASR) systems have been gaining popularity in the recent years for their widespread usage in smart phones and speakers. Building ASR systems for task-specific scenarios is subject to the availability of utterances that adhere to the style of the task as well as the language in question. In our work, we target such a scenario wherein task-specific text data is available in a language that is different from the target language in which an ASR Language Model (LM) is expected. We use Neural Machine Translation (NMT) as an intermediate step to first obtain translations of the task-specific text data. We then train LMs on the 1-best and N-best translations and study ways to improve on such a baseline LM. We develop a procedure to derive word confusion networks from NMT beam search graphs and evaluate LMs trained on these confusion networks. With experiments on the WMT20 chat translation task dataset, we demonstrate that NMT confusion networks can help to reduce the perplexity of both n-gram and recurrent neural network LMs compared to those trained only on N-best translations.

==> acknowledgements/acknowledgements.tex <==
\cleardoublepage

\addcontentsline{toc}{chapter}{Acknowledgements}

\begin{acknowledgements}

This thesis would not have been possible without the support of many people in the extra-ordinary times of the pandemic.

First and foremost, I would like to thank my supervisor Juan Ye for many things. Not only did you  introduce me to the field of lifelong learning but also granted me the freedom to pursue my research in the direction I wanted to. I can admissibly claim that I have been on the pinnacle of resourcefulness during the last six months. 


I also owe my deepest appreciations to Martin Schiemer who has been there guiding me since day one. Thank you Martin for bearing the migraines of hours of debugging to find those missing semicolons! It indeed were Juan and Martin who \textit{continually} flooded me with wonderful advice for the thesis across the span of the semester.


Having carried out most of my thesis work in the tough times of social distancing, I am grateful to the \textit{incremental} support I received from my fellow Masters' friends in St Andrews (in alphabetical order): Aniruddh, Azamat, Balint, Gunay, Giorgio, Hassan, Katerina, Marika, Neha, Oskar, Priyam, Ritomo, Sakina, Sergio, Shamsiddin and Shubham. Scotland would never be so beautiful without you. Further thanks to Kunal, Pawan and Vijay for making me feel homely throughout the lockdown.

My biggest shoutout goes to my parents, my brother and my sister who have been my source of \textit{lifelong} encouragement in everything I do and every decision I make. Dear mom and dad, all this would have no chance of becoming true had you not helped me pursue my engineering dream.

Finally, thank you Erasmus Mundus for offering such generous scholarships that has allowed me and thousands of others like me to pursue our dream of European Masters while shaping our international careers across highly reputed universities. Thanks too to my uncle Ajit who was forever encouraging me to apply for EMJMD.
\end{acknowledgements}
